Polynomial Neural Fields for Subband Decomposition and Manipulation

Neural fields have emerged as a new paradigm for representing signals, thanks to their ability to do it compactly while being easy to optimize. In most applications, however, neural fields are treated like black boxes, which precludes many signal manipulation tasks. In this paper, we propose a new class of neural fields called polynomial neural fields (PNFs). The key advantage of a PNF is that it can represent a signal as a composition of a number of manipulable and interpretable components without losing the merits of neural fields representation. We develop a general theoretical framework to analyze and design PNFs. We use this framework to design Fourier PNFs, which match state-of-the-art performance in signal representation tasks that use neural fields. In addition, we empirically demonstrate that Fourier PNFs enable signal manipulation applications such as texture transfer and scale-space interpolation. Code is available at https://github.com/stevenygd/PNF.

==> figures/all_sdfs/fig.tex <==
\begin{figure*}[htb!]
\centering
\begin{minipage}{\textwidth}

\begin{minipage}{.4\textwidth}
  \centering
    \includegraphics[width=0.25\textwidth]{figures/sdfs_qualitative/pnf-sdf-comparison-fs8.png}
    \caption{CAPTION: Shape fitting with}
    \label{fig:shapefitting}
\end{minipage}

\begin{minipage}{.25\textwidth}
\centering
\includegraphics[width=\linewidth]{figures/convergence/thai_sdf_convergence.pdf}
\caption{Convergence comparison for selected shapes from the Stanford 3D scanning repository. x-axis shows the number of steps (K) and the y-axis shows the validation chamfer distance (multiplied by $10^6$) }
\centering
\caption{Evaluation for fitting the 3D shape of \textit{thai}. CD stands for chamfer distance (multiplied by $10^{6}$) and FS stands for F-score (in \%)}
\begin{tabular}{@{}lcc@{}}
\toprule
              &   \multicolumn{1}{l}{CD $\downarrow$ } & \multicolumn{1}{l}{FS $\uparrow$} \\ \midrule
SIREN            & \multicolumn{1}{r}{9.00}        & \multicolumn{1}{r}{99.76\%} \\
BACON            & \multicolumn{1}{r}{2.60}        & \multicolumn{1}{r}{99.84\%} \\
BACON-L       & \multicolumn{1}{r}{2.60}        & \multicolumn{1}{r}{99.85\%} \\
BACON-M       & \multicolumn{1}{r}{2.61}        & \multicolumn{1}{r}{99.85\%} \\              \\
PNF    & \multicolumn{1}{r}{\textbf{2.25}}	 &  \multicolumn{1}{r}{\textbf{99.97\%}}                   \\
\midrule
Oracle           & \multicolumn{1}{r}{2.35}           & \multicolumn{1}{r}{100\%} \\ \bottomrule
\end{tabular}
\label{tab:sdf}

\end{minipage}%

\begin{minipage}{.34\textwidth}
\end{minipage}%

\end{minipage}
\end{figure*}

==> figures/convergence/fig.tex <==
\begin{minipage}[t]{0.45\textwidth}
\centering
\centering
\includegraphics[width=1.0\linewidth]{figures/convergence/thai_sdf_convergence.pdf}
\vspace{-0.2cm}
\caption{3D shape fitting convergence comparison. x-axis is the number of steps (K) and the y-axis is the validation Chamfer Distance ($\times 10^6$) \sagie{MAKE THIS ONE FIG}(a and b)}
\label{fig:sdf-convergence}
\end{minipage}%

==> figures/freq_subband/freq_subband.tex <==

\begin{figure*}
    \centering
    \includegraphics[width=0.36\linewidth]{figures/freq_subband/subbands.pdf}
    \includegraphics[width=0.55\linewidth]{figures/freq_subband/fourier-PNF.pdf}
    \vspace{-0.5em}
    \caption{Left figure shows instances of two types of Fourier subbands and how these subbands tile the space. The right figure illustrate the architecture of $F_i$(\cref{eq:ff-pnf-within-set}), a part of Fourier-PNF operates within a controllable set of subband. The output of Fourier PNF is an ensemble of these networks.}
    \label{fig:architecture}
\end{figure*}

==> figures/laplacian_supp2/fig.tex <==
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\begin{figure*}
\begin{center}
\begin{tabular}{c@{}c@{}c@{}c@{~~~}c@{}c@{}c@{}c@{}c}
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_gau_0.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_lap_1.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_lap_2.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_lap_3.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_gau_0.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_lap_1.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_lap_2.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_lap_3.png} \\

\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_gau_0.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_gau_1.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_gau_2.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/bacon/05_BACON_log_quant_last_gau_3.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_gau_0.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_gau_1.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_gau_2.png} &
\includegraphics[width=0.12\linewidth,height=0.12\linewidth]{figures/laplacian_supp2/pnf/05_pnf_PNF_pseudopolar_fix2_gau_3.png}
 \\
 \multicolumn{4}{c}{BACON} & \multicolumn{4}{c}{PNF}
\end{tabular}
\caption{BACON: The bottom row shows the output of each layer which is upper band limited. The top row (columns 2-4) shows the difference between the output of a given layer and the one before it. PNF: The top row shows the output of each layer which is both upper and lower band limited. The bottom row (columns 2-4) shows the addition of the output at a given layer and the one before it. }
\label{fig:laplacian-pyramid_supp2}
\end{center}
\end{figure*}

==> tables/parameter-efficiency.tex <==
\centering
\caption{A comparison of the number of parameters used for experiments conduced to asses expressivity in \cref{sec:expressivity}. One the right, we consider the type of experiment conducted: neural fields (NeRF - 1x to 1/8x resolution), image fitting (Image) and 3D signed distance field (SDF).  On the rows, we consider our method in comparison to baselines.  }
\begin{tabular}{lcccc}
\toprule
Experiment & PNF (Our) & BACON & RFF & SIREN \\ 
\midrule
NeRF 1x & 0.46M & 0.54M & - & - \\ 
NeRF 1/2x & 0.34M & 0.41M  & - & -  \\ 
NeRF 1/4x & 0.23M & 0.27M  & - & - \\ 
NeRF 1/8x  & 0.12M & 0.14M & - & - \\  
Image & 0.28M & 0.27M  & 0.26M & 0.26M \\
SDF & 0.59M & 0.54M & - & 0.53M  \\		
\bottomrule
\label{tab:param_efficiency}
\end{tabular}
